BOBA: A Parallel Lightweight Graph Reordering Algorithm with Heavyweight Implications

We describe a simple parallel-friendly lightweight graph reordering algorithm for COO graphs (edge lists). Our ``Batched Order By Attachment'' (BOBA) algorithm is linear in the number of edges in terms of reads and linear in the number of vertices for writes through to main memory. It is highly parallelizable on GPUs\@. We show that, compared to a randomized baseline, the ordering produced gives improved locality of reference in sparse matrix-vector multiplication (SpMV) as well as other graph algorithms. Moreover, it can substantially speed up the conversion from a COO representation to the compressed format CSR, a very common workflow. Thus, it can give \emph{end-to-end} speedups even in SpMV\@. Unlike other lightweight approaches, this reordering does not rely on explicitly knowing the degrees of the vertices, and indeed its runtime is comparable to that of computing degrees. Instead, it uses the structure and edge distribution inherent in the input edge list, making it a candidate for default use in a pragmatic graph creation pipeline. This algorithm is suitable for road-type networks as well as scale-free. It improves cache locality on both CPUs and GPUs, achieving hit rates similar to the heavyweight techniques (e.g., for SpMV, 7--52\% and 11--67\% in the L1 and L2 caches, respectively). Compared to randomly labeled graphs, BOBA-reordered graphs achieve end-to-end speedups of up to 3.45. The reordering time is approximately one order of magnitude faster than existing lightweight techniques and up to 2.5 orders of magnitude faster than heavyweight techniques.

==> tex/acknowledgments.tex <==

%% Acknowledgments
\begin{acks}                            %% acks environment is optional
    %% contents suppressed with 'anonymous'
%% Commands \grantsponsor{<sponsorID>}{<name>}{<url>} and
%% \grantnum[<url>]{<sponsorID>}{<number>} should be used to
%% acknowledge financial support and will be used by metadata
%% extraction tools.
This material is based upon work supported by the
\grantsponsor{GS100000001}{National Science
Foundation}{http://dx.doi.org/10.13039/100000001} under Grant
No.~\grantnum{GS100000001}{nnnnnnn} and Grant
No.~\grantnum{GS100000001}{mmmmmmm}.  Any opinions, findings, and
conclusions or recommendations expressed in this material are those
of the author and do not necessarily reflect the views of the
National Science Foundation.

Lars Nyland, NVIDIA
Any NV/RAPIDS folks who offered advice
\end{acks}


==> tex/model.tex <==
\section{An Optimization Problem}
\label{sec:analysis}

\citet{Wei:2016:SGP} formulate the graph reordering problem as an instance of \textsc{TSP}:
\[
    \begin{aligned}
        \textsc{$\text{GScore}$} &  & \max        & \sum_{ij \in [n]^2}s_{ij}x_{ij}                            \\
                                 &  & \text{s.t.} & \sum_{j > i}x_{ij} + \sum_{i < j}x_{ji} = 2 & i,j \in [n]  \\
                                 &  &             & x_{ij} \in \{0,1\}                          & i,j \in [n].
    \end{aligned}
\]
Here $s_{ij} := |N(v_i) \cap N(v_j)|$.
We can think of $x_{ij}$ indicating whether $v_iv_j$ appears in a corresponding feasible solution for \textsc{TSP}. A $\frac{1}{2}$-approximation algorithm is given in \cite{Wei:2016:SGP}, which runs in time $O(\deg_{\max}(v)n^2)$.

We show that under the \textsc{LCD} model of \citet{Bollobas:2004:TDO} that simply ordering vertices by arrival time gives a constant factor approximation to \textsc{GScore}.

\subsection{Preferential Attachment and LCD model}

\subsection{Approximation Algorithm}


